A 2D Parallel Triangle Counting Algorithm for Distributed-Memory Architectures

Triangle counting is a fundamental graph analytic operation that is used extensively in network science and graph mining. As the size of the graphs that needs to be analyzed continues to grow, there is a requirement in developing scalable algorithms for distributed-memory parallel systems. To this end, we present a distributed-memory triangle counting algorithm, which uses a 2D cyclic decomposition to balance the computations and reduce the communication overheads. The algorithm structures its communication and computational steps such that it reduces its memory overhead and includes key optimizations that leverage the sparsity of the graph and the way the computations are structured. Experiments on synthetic and real-world graphs show that our algorithm obtains an average relative speedup that range between 3.24 and 7.22 out of 10.56 across the datasets using 169 MPI ranks over the performance achieved by 16 MPI ranks. Moreover, we obtain an average speedup of 10.2 times on comparison with previously developed distributed-memory parallel algorithms.

==> ack.tex <==
% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi
\noindent
This work was supported in part by NSF (1447788, 1704074, 1757916, 1834251), Army
Research Office (W911NF1810344), Intel Corp, and the Digital Technology Center at the
University of Minnesota. Access to research and computing facilities was provided by
the Digital Technology Center and the Minnesota Supercomputing Institute.

==> nodespercore.tex <==
\begin{table}[h]
  \small
  \centering
  \begin{threeparttable}
    \caption{Number of nodes used for varying number of ranks in the algorithm.}
    \label{table:nodespercore}
%    \begin{tabular}{|L{2cm}|R{2cm}|R{2cm}|}
    \begin{tabular}{|l|r|r|r|}
      \toprule
      \midrule
%      \multicolumn{1}{|c|}{} 		& \multicolumn{1}{c|}{fastest} 			&   \\
      \multicolumn{1}{|c|}{} 		& \multicolumn{1}{c|}{fastest runtime} 	&  \multicolumn{1}{c|}{cores} & \multicolumn{1}{c|}{speedup}\\
      \multicolumn{1}{|c|}{Graph} &  \multicolumn{1}{c|}{reported (in sec)} 		&  \multicolumn{1}{c|}{used} & \multicolumn{1}{c|}{achieved}\\
      \midrule
	Our work									& 46.9	& \textcolor{red}{100} 	&  - \\
	AOP~\cite{arifuzzaman2017distributed}			& 564.0	& 200	&  12.0$\times$\\
	Surrogate~\cite{arifuzzaman2017distributed}		& 739.8	& 200	&  15.7$\times$ \\
	HavoqGT~\cite{6569865}						& 511.2	& 6144	&  10.9$\times$\\
	OPT-PSP~\cite{kanewala2018distributed}			& 		&  		&\\
      \bottomrule
    \end{tabular}
    \begin{tablenotes}
    \footnotesize
        \item We make comparisons with four competing approaches on the \emph{twitter} dataset.
    	\item We make use of the fastest runtimes (in seconds) reported in~\cite{arifuzzaman2017distributed, kanewala2018distributed, 6569865} and also report the number of cores they used in obtaining the runtimes.
	\iffalse
	\begin{enumerate}
    		\item Algorithm with Overlapping Partitioning (AOP)~\cite{arifuzzaman2017distributed}, run on 200 cores.
    		\item Surrogate~\cite{arifuzzaman2017distributed} run on 200 cores.
		\item HavoqGT~\cite{6569865} run on 256 nodes with 24 cores each.
		\item OPT-PSP algorithm~\cite{kanewala2018distributed} (extrapolate numbers?) run on 64 cores.
	\end{enumerate}
	\fi
    \end{tablenotes}   
  \end{threeparttable}
\end{table}
